Language Models as Few-Shot Learner for Task-Oriented Dialogue Systems

Task-oriented dialogue systems use four connected modules, namely, Natural Language Understanding (NLU), a Dialogue State Tracking (DST), Dialogue Policy (DP) and Natural Language Generation (NLG). A research challenge is to learn each module with the least amount of samples (i.e., few-shots) given the high cost related to the data collection. The most common and effective technique to solve this problem is transfer learning, where large language models, either pre-trained on text or task-specific data, are fine-tuned on the few samples. These methods require fine-tuning steps and a set of parameters for each task. Differently, language models, such as GPT-2 (Radford et al., 2019) and GPT-3 (Brown et al., 2020), allow few-shot learning by priming the model with few examples. In this paper, we evaluate the priming few-shot ability of language models in the NLU, DST, DP and NLG tasks. Importantly, we highlight the current limitations of this approach, and we discuss the possible implication for future work.

==> IMG.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,485); %set diagram left start at 0, and has height of 485

%Rounded Rect [id:dp06582212785349983] 
\draw  [fill={rgb, 255:red, 254; green, 184; blue, 197 }  ,fill opacity=1 ] (411,155.73) .. controls (411,152.57) and (413.57,150) .. (416.73,150) -- (595.93,150) .. controls (599.1,150) and (601.67,152.57) .. (601.67,155.73) -- (601.67,172.93) .. controls (601.67,176.1) and (599.1,178.67) .. (595.93,178.67) -- (416.73,178.67) .. controls (413.57,178.67) and (411,176.1) .. (411,172.93) -- cycle ;
%Straight Lines [id:da6009740910999917] 
\draw    (505,124.67) -- (505,144) ;
\draw [shift={(505,146)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7434991855797852] 
\draw    (505,184.67) -- (505,204) ;
\draw [shift={(505,206)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (464.33,214) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{54.378784pt}\setlength\topsep{0pt}
\begin{center}
$ ${\fontfamily{pcr}\selectfont light\_on }
\end{center}

\end{minipage}};
% Text Node
\draw (506.33,164.33) node   [align=left] {{\fontfamily{pcr}\selectfont Language Model(GPT)}};
% Text Node
\draw (383.33,13.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{165.75pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{pcr}\selectfont turn on the light}{\fontfamily{ptm}\selectfont  }$\displaystyle \ \rightarrow ${\fontfamily{ptm}\selectfont  }{\fontfamily{pcr}\selectfont light\_on \textbackslash n }\\{\fontfamily{pcr}\selectfont turn off the light}{\fontfamily{ptm}\selectfont  }$\displaystyle \rightarrow ${\fontfamily{ptm}\selectfont  }{\fontfamily{pcr}\selectfont light\_off\textbackslash n}\\$\displaystyle \cdots $\\{\fontfamily{pcr}\selectfont light on, please}{\fontfamily{ptm}\selectfont  }$\displaystyle \rightarrow ${\fontfamily{ptm}\selectfont  }
\end{center}

\end{minipage}};


\end{tikzpicture}

